THOS: A Benchmark Dataset for Targeted Hate and Offensive Speech

Detecting harmful content on social media, such as Twitter, is made difficult by the fact that the seemingly simple yes/no classification conceals a significant amount of complexity. Unfortunately, while several datasets have been collected for training classifiers in hate and offensive speech, there is a scarcity of datasets labeled with a finer granularity of target classes and specific targets. In this paper, we introduce THOS, a dataset of 8.3k tweets manually labeled with fine-grained annotations about the target of the message. We demonstrate that this dataset makes it feasible to train classifiers, based on Large Language Models, to perform classification at this level of granularity.

==> icml2023/LimitationAndFutureWork.tex <==
\section{Limitations and Future Work}
\label{sec:LaFW}
\textbf{Limitations}: In our work, we have focused on the speech's type and the speech's target. However, considering other factors such as the context (i.e. replies) and its sentiment might improve the model's performance. Also, our work focuses on a single language. The translation to help the model to classify other languages is not enough since the hate speech (i.e. implicit hate speech) classification mostly relies more on the culture and environment than the text's lexical meaning.

\textbf{Future Work}: In the first experiment, the TPCs classification where getting more high results than STPCs. Meanwhile, the STPCs classification has been improved while providing the TPCs as input features. So, using multi-task learning might be a good direction for the classification task. Also, considering the tweet context (i.e. replies) might be a good direction for implicit hate speech detection. The results show that the topics and subtopics can slightly improve the hate speech classification.
